GQA: A New Dataset for Real-World Visual Reasoning and Compositional Question Answering

We introduce GQA, a new dataset for real-world visual reasoning and compositional question answering, seeking to address key shortcomings of previous VQA datasets. We have developed a strong and robust question engine that leverages scene graph structures to create 22M diverse reasoning questions, all come with functional programs that represent their semantics. We use the programs to gain tight control over the answer distribution and present a new tunable smoothing technique to mitigate question biases. Accompanying the dataset is a suite of new metrics that evaluate essential qualities such as consistency, grounding and plausibility. An extensive analysis is performed for baselines as well as state-of-the-art models, providing fine-grained results for different question types and topologies. Whereas a blind LSTM obtains mere 42.1%, and strong VQA models achieve 54.1%, human performance tops at 89.3%, offering ample opportunity for new research to explore. We strongly hope GQA will provide an enabling resource for the next generation of models with enhanced robustness, improved consistency, and deeper semantic understanding for images and language.

==> analysis-copy.tex <==
\section{Analysis and Baseline experiments}
%\label{sec:exps}
% continue motivation 

% analyze the resultant dataset and compare it with existing benchmarks. We present and discuss the new metrics and use them to evaluate an array of baselines and state-of-the-art models, comparing them to human subjects and revealing a large gap in performance across multiple axes. Finally, we discuss models' strengths and weakness discovered through the analysis on GQA, and propose potential research directions to overcome them.
% across multiple axes
In the following, we provide an analysis of the GQA dataset, perform a head-to-head comparison with the popular VQA 2.0 dataset \cite{vqa2}, and evaluate the performance of baselines, state-of-the-art models and human subjects, revealing a large gap from the latter. To establish the diversity and realism of GQA questions, we then show test transfer performance between the GQA and VQA datasets. We then introduce the new metrics that complement our dataset, present quantitative results and discuss their implications and merits. In the supplementary, we proceed with further diagnosis of the current top-performing model, MAC \cite{mac}, evaluating it along multiple axes such as training-set size, question length and compositionality degree.   

% clevr human in performance in performance between the formers and 
%While CLEVR questions are longer on average, they refer to artificial images  As shown in figure XXX, 

\subsection{Dataset Analaysis and Comparison}
\label{sec:analysis}

%cake for steps, fix cake 

% , XXX of them are unique The short-answer length matches those of other datasets, while the long answer provides more detail and justification. GQA has the ones in the note that \eg 82\% of the VQA2.0 questions have in fact answers among the top 1000k \cite{visual7w}. F
% While GQA has a smaller question and answer vocabulary than VQA, 
 
The GQA dataset includes 22,669,678 questions over 113,018 images. As \figref{distt} shows, the questions tend to longer than those of the VQA2.0 benchmark, alluding to their higher compositionality degree (\figref{cakes}). It has a vocabulary size of 3097 words and 1878 possible answers. While inadvertently smaller than natural language datasets, further investigation reveals that it covers 88.8\% and 70.6\% of VQA questions and answers respectively, corroborating its wide diversity. A wide selection of dataset visualizations is provided in the supplementary.
% the   vary greatly in lengths, commonly 

We associate each question with two types: structural and semantic. The \textbf{structural type} is derived from the final operation in the question's functional program. It can be (1) \textbf{verify} for yes/no questions, (2) \textbf{query} for all open questions, (3) \textbf{choose} for questions that present two alternatives to choose from, \eg \textit{``Is it red or blue?";} (4) \textbf{logical} which involve logical inference, and (5) \textbf{compare} for comparison questions between two or more objects. The \textbf{semantic type} refers to the main subject of the question: (1) \textit{object}: for existence questions, (2) \textit{attribute}: consider the properties or  position of an object, (3) \textit{category}: related to object identification within some class, (4) \textit{relation}: for questions asking about the subject or object of a described relation (\eg \textit{``what is the girl wearing?"}), and (5) \textit{global}: about overall properties of the scene such as weather or place. As shown in \figref{cakes}, the questions have diverse set of types in both the semantic and structural levels.

% verification pertaining to the existence of an object, attribute or relation
% as well as  , including \eg \textit{or}, \textit{and} or \textit{not}; for questions for questions that for questions spatial  the structural levels a structural type and a semantic type for questions that \dots 

% 
% examination wide \footnote{In this version of the dataset, we avoid generation of counting questions since oftentimes for images with many objects of the same type, such as animals in a herd or an assortment of vegetables, the existing scene graphs do not provide exhaustive coverage of all the object instances, or group them together into one plural object, \eg \textit{horses}. However, if additional annotations are provided, GQA can be easily extended to include such questions as well.} 

% ADDBACK
% We proceed by performing a comparison with the VQA 2.0 dataset \cite{vqa2}, the findings of which are summarized in table \ref{table1}. Apart from the higher average question length, we can see that GQA consequently contains more verbs and prepositions than VQA (as well as more nouns and adjectives), providing further evidence for its increased compositionality. Semantically, we can see that the GQA questions are significantly more compositional than VQA's, and involve variety of reasoning skills in much higher frequency (spatial, logical, relational and comparative).
% further from the table  head-to-head 

% Some VQA question types are not covered by GQA, such as intention (\textit{why}) questions or ones involving OCR or external knowledge. The GQA dataset focuses on factual questions and multi-hop reasoning in particular, rather than covering all types. Comparing to VQA, GQA questions are objective, unambiguous, more compositional and can be answered from the images only, potentially making this benchmark more controlled and convenient for making research progress on. 
% Overall, we see the GQA and VQA datasets as complementary rather than alternatives, testing together a wide range of intellectual skills.
%  accuracy quite good achieves
% Following reviewers' suggestions, we performed transfer experiments between GQA and VQA, training on the one and testing on the other: a MAC model
%The reviewers have asked about transfer results between GQA and VQA datasets, \ie training on the one and testing on the other. 
%and the results are the following
% they are We can see that 
% both before and after fine-turning. The results 
% the ability to answer 
% beyond VQA, \ie baseline an the dataset suggestions  that was the We see that the transfer results are quite good, and 



% in particular over

% lingustic-style comparison + smaller vocab is actually good, isolate the problem

%To asses the diversity 
% We have trained the models on the train set and report all the results on test-dev set.
 
\subsection{Baseline Experiments}
\label{sec:exps}
\begin{table}
\scriptsize 
\begin{center}
\begin{tabular}{lcc}
\rowcolor{Blue1}
\textbf{Aspect} & \textbf{VQA} & \textbf{GQA} \\
Question length & 6.2 + 1.9 & 7.9 + 3.1 \\
\rowcolor{Blue2}
Relation questions & 19.5\% & 51.6\% \\
Spatial questions & 8\% & 22.4\% \\
\rowcolor{Blue2}
Logical questions & 6\% & 19\% \\
Comparative questions & 1\% & 3\% \\
\rowcolor{Blue2}
Compositional questions & 3\% & 52\% \\
\end{tabular}
\end{center}
\caption{A comparison between GQA and VQA 2.0. GQA questions are longer on average, more compositional and require more reasoning: spatial, logical, relational, comparative.}

\label{table1}
\end{table}

% most likely explore evaluate , including baselines as well as state-of-the-art models
We analyse an assortment of models as well as on human subjects on the GQA. Baselines include a ``blind" LSTM model with access to the questions only, a ``deaf" CNN model with access to the images only, an LSTM+CNN model, and two prior models based on the question group, local or global, which return the most common answer for each group, as defined in \secref{exppp}. Beside these, we evaluate the performance of the bottom-up attention model \cite{bottomup} -- the winner of 2017 VQA challenge, and the MAC model \cite{mac} -- a compositional attention state-of-the-art model for CLEVR \cite{clevr}. For human evaluation, we used Amazon Mechanical Turk to collect human responses for 4000 random questions, taking majority over 5 answers per question. Further description of the evaluated models along with implementation details can be found in the supplementary. 
% Besides, hyperparameter values and 

The evaluation results, including the overall accuracy and the accuracies for each question type, are summarized in table \ref{table2}. As we can see, the priors and the blind LSTM model achieve very low results of 41.07\%: inspection of specific question types reveals that LSTM achieves only 22.7\% for open \textit{query} questions, and not far above chance for all other binary question types. We can further see that the ``deaf" CNN model achieves as well low results across almost all question types, as expected. On the other hand, state-of-the-art models such as MAC \cite{mac} and Bottom-Up Attention \cite{bottomup} perform much better than baselines, but still well below human scores, offering ample opportunity for further research in the visual reasoning domain.

% Notebly, they achieve quite high results for object questions, which indeed are conditioned on the identity of each object, and thus can adapt to its unique distribution. For CNN, the results may indicate that it can ``guess" the correct object, by looking at the main entities in the image, an intuitive observation that the experiments confirm. 

% experimented
% \footnotetext{\label{note1}In a previous version we computed validity, plausibility and consistency in a different way, leading to lower scores than those reported here.}

% The previous version of the paper
%recall.. Notebly every concept is once -> for acc
% acountable In the spirit, cogent are using
% shed more light on models performance capabilities we believe coherent reasoning models should demonstrate by inspecting the 
% \subsection{Transfer Performance}

% ADDBACK
% The GQA questions are longer on average, and consequently have more verbs, nouns, adjectives and prepositions than VQA, alluding to their increased compositionality. In addition, GQA demands increased reasoning (spatial, logical, relational and comparative) and includes significantly more compositional questions.

% ADDBACK
\subsection{Transfer Performance}
We tested the transfer performance between the GQA and VQA datasets, training on one and testing on the other: A MAC model trained on GQA achieves 52.1\% on VQA before fine-tuning and 60.5\% afterwards. Compare these with 51.6\% for LSTM+CNN and 68.3\% for MAC, when both are trained and tested on VQA. These quite good results demonstrate the realism and diversity of GQA questions, showing the dataset can serve as a good proxy for human-like questions. In contrast, MAC trained on VQA gets 39.8\% on GQA before fine-tuning and 46.5\% afterwards, illustrating the further challenge GQA poses.

\subsection{New Evaluation Metrics}
\label{sec:metrics}

\begin{table*}
\centering
\scriptsize 
\begin{tabular}{lcccccccc}
\rowcolor{Blue1}
\scriptsize \textbf{Metric} & \textbf{Global Prior} & \textbf{Local Prior} & \textbf{CNN} & \textbf{LSTM} & \textbf{CNN+LSTM} & \textbf{BottomUp} & \textbf{MAC} & \textbf{Humans} \\ 
Open & 
16.52 &
16.99 &
1.74	 &
22.69 &
31.80 &
34.83 &
38.91 & 87.4 \\[0.2em] 

Binary &
42.99 &
47.53 &
36.05 &
61.90 &
63.26 &
66.64 &
71.23 & 91.2 \\[0.2em] % mac 0.535767512347627

\rowcolor{Blue2}
Query &
16.52 &
16.99 &
1.55 &
22.69 &
31.80 &
34.83 &
38.91 & 87.4 \\[0.2em] % mac query 0.3863219539343039

\rowcolor{Blue2}
Compare &
35.59 &
41.91 &
36.34 &
57.79 &
56.62 &
56.32 &
60.04 & 93.1\\[0.2em] % mac compare 0.6813143309580364

\rowcolor{Blue2}
Choose &
17.45 &
26.58 &
0.85 &
57.15 &
61.40 &
66.56 &
70.59 & 94.3\\[0.2em] % mac choose 0.7492180607907611

\rowcolor{Blue2}
Logical &
50.32 &
50.11 &
47.18 &
61.73 &
62.05 &
64.03 &
69.99 & 88.5 \\[0.2em] % mac logical 0.8142637565324315

\rowcolor{Blue2}
Verify &
53.40 &
58.80 &
47.02 &
65.78 &
67.00 &
71.45 &
75.45 & 90.1 \\[0.2em] % mac verify 0.7193132314000171

Global &
24.70 &
20.19 &
8.64 &
27.22 &
56.57 &
60.29 &
60.82 & 92.3 \\[0.2em] % mac global 0.5955941794664511

Object &
49.96 &
54.00 &
47.33 &
74.33 &
75.90 &
78.45 &
81.49 & 88.1 \\[0.2em] % mac obj 0.8061453172918142

Attribute &
34.89 &
42.67 &
22.66 &
48.28 &
50.91 &
53.88 &
59.82 & 90.7\\[0.2em] % mac attr 0.6102285826749515

Relation &
22.88 &
20.16 &
11.60 &
33.24 &
39.45 &
42.84 &
46.16 & 89.2 \\[0.2em] % mac rel 0.42713495447735395

Category &
15.26 &
17.31 &
3.56 &
22.33 &
37.49 &
41.18 &
44.38 & 90.3 \\[0.2em] % mac cat 0.5806486025176019 \\[1ex]	

\rowcolor{Blue2}
Distribution &
130.86 &
21.56 &
19.99 &
17.93 &
7.46 &
5.98 &
5.34 & - \\[0.2em]

Grounding &
- &
- &
- &
- &
- &
78.47 &
82.24 & - \\[0.2em]			

\rowcolor{Blue2}
Validity &%\footnotemark[13]
89.02 &
84.44 &
35.78 &
96.39 &
96.02 &
96.18 &
96.16 & 98.9 \\[0.2em] % mac 0.9029803098465445

\rowcolor{Blue2}
Plausibility &%\footnotemark[13]
75.34 &
84.42 &
34.84 &
87.30 &
84.25 &
84.57 &
84.48 & 97.2 \\[0.2em] % mac 0.46709623443244946

Consistency &%\footnotemark[13]
51.78 &
54.34 &
62.40 &
68.68 &
74.57 &
78.71 &
81.59 & 98.4 \\[0.2em] % mac 0.5940163485139546

\rowcolor{Blue2}
\textbf{Accuracy} &
\textbf{28.93} &
\textbf{31.31} &
\textbf{17.82} &
\textbf{41.07} &
\textbf{46.55} &
\textbf{49.74} &
\textbf{54.06} & \textbf{89.3} \\[0.2em] % mac 0.535767512347627

%  sptial 42.97 objects 
\end{tabular}
\vspace*{2mm}
\caption{Results for baselines and state-of-the-art models on the GQA dataset. All results refer to the test set. Models are evaluated for overall accuracy as well as accuracy per type. In addition, they are evaluated by validity, plausibility, distribution, consistency, and when possible, grounding metrics. Please refer to the text for further detail.}
\label{table2}
\end{table*}

% ADDBACK !!!
% \begin{figure}
% \centering
% \subfloat{\includegraphics[width=\linewidth]{imgs/qdist.pdf}}
% \caption{Question length distribution for Visual Question Answering datasets: we can see that GQA questions have a wide range of lengths and are longer on average than all other datasets except the synthetic CLEVR. Note that the long CLEVR questions tend to sound unnatural at times. }
% \label{fig:distt}
% \end{figure}

Apart from the standard accuracy metric, and the more detailed type-based diagnosis our dataset supports, we introduce five new metrics to get further insight into visual reasoning methods and point to missing capabilities we believe coherent reasoning models should possess. 

%  -- whether or not contradictory answers are given to equivalent or entailed questions We compute this metric by averaging over the accuracy of all the entailed questions of a source question $q$, given that it was answered correctly.  performance and The first metric measures the level of the 
\textbf{Consistency}. measure responses consistency across different questions. Recall that in  \secref{exppp}, we used the questions' semantic representation to derive equivalence and entailment relations between them. When being presented with a new question, any learner striving to be trustworthy should not contradict its previous answers. It should not answer ``green" to a new question about an apple it has just identified as ``red". 

For each question-answer pair $(q,a)$, we define a set $E_q={q_1, q_2, \dots, q_n}$ of entailed questions, the answers to which can be unambiguously inferred given $(q,a)$. For instance, given the question-answer pair \textit{``Is there a red apple to the left of the white plate?"}, we can infer the answers to questions such as \textit{Is the plate to the right of the apple?}, \textit{``Is there a red fruit to the left of the plate?"}, \textit{``What is the white thing to the right of the apple?"}, etc. For each question $q$ in $Q$ -- the set of questions \textit{the model answered correctly}, we measure the model's accuracy over the entailed questions $E_q$ and then average these score across all questions in $Q$. 
% Denote $Q$ the set of all questions . to get the score $s_q$ 

% robust to? with state-of-the-are models achieving better scores than the baselines. 
We can see that while people have exceptional consistency of 98.4\%, even best models are inconsistent in about 1 out of 5 questions, and models such as LSTM contradict themselves almost half the times. Apparently, achieving high consistency requires deeper understanding of the question semantics in the context of the image, and, in contrast with accuracy, is more robust against ``random" educated guesses as it inspects connections between related questions, and thus may serve as a better measure of models' true visual understanding skills.

% The results also show that models frequently fail to be \textit{consistent}, replying with contradictory answers to equivalent or entailed questions.

%  (for at least some images the most-common answer 
% Second, the \textbf{validity} metric measures the extent to which a model's response is in the scope of theoretically-possible answers to a given question for at least some images, \eg responding some color to a color question. For instance, if a question asks whether a color of an apple is red or green, only these two alternative are valid answers. a model's
% of theoretically-possible answers to a given, defined by 
% latter quantifies the degree to which the measures the extent to which the model's \text to given questions and so capture well at least the general tendencies of the dataset to the presented questions, question-, former, latter

\begin{figure}
\vspace*{-2mm}
\centering
\subfloat{\includegraphics[width=0.35\linewidth]{imgs/cakenew1.pdf}}
\subfloat{\includegraphics[width=0.325\linewidth]{imgs/cakenew2.pdf}}
\subfloat{\includegraphics[width=0.335\linewidth]{imgs/cake3.pdf}}

\caption{Dataset statistics: partitioned into structural types -- the final operation to be performed, semantic types -- the main subject of the question, and the number of reasoning steps.}
\label{fig:cakes}
\label{fig:distt}
\end{figure}
% : we can see that GQA questions have a wide range of lengths and are longer on average than all other datasets except the synthetic CLEVR. Note that the long CLEVR questions tend to sound unnatural at times. 

\textbf{Validity} and \textbf{Plausibility}. The validity metric checks whether a given answer is in the scope of the question, \eg responding some color to a color question. The plausibility score goes a step further, measuring whether the answer is reasonable, or makes sense, given the question (\eg elephant usually do not eat, say, pizza). Specifically, we check whether the answer occurs at least once in relation with the question's subject, across the whole dataset, thus, for instance, we consider \eg \textit{red} and \textit{green} as plausible apple colors, wheres \textit{purple} as not.\footnote{While the plausibility metric may not be fully precise especially for infrequent objects due to potential data scarcity issues, it may provide a good sense of the general level of world-knowledge the model has acquired.} The experiments show that models fail to respond with plausible or even valid answers in at least 5-15\% of the times, indicating limited comprehension of some questions. Given that these properties are noticeable statistics of the dataset's conditional answer distribution, not even depending on the specific images, we would expect a sound method to achieve higher scores.

% degree, enhacned, refined 
\textbf{Distribution}. To get further insight into the extent to which methods manage to model the conditional answer distribution, we define the distribution metric, which measures the overall match between the true answer distribution and the model predicted distribution. For each question global group (\secref{exppp}), we compare the golden and prediction distributions using Chi-Square statistic \cite{chisquare}, and then average across all the groups. It allows us to see if the model predicts not only the most common answers but also the less frequent ones. Indeed, the experiments demonstrate that better models such as the state-of-the-art Bottom Up and MAC models score lower than the baselines (for this metric, lower is better), indicating increased capacity in fitting more subtle trends of the dataset's distribution. 

% is relevant to answer it (or alternatively, multiple pointers to relevant regions) validate usefulness discerment
\textbf{Grounding}. For attention-based models, the grounding score checks whether the model attends to regions within the image that are relevant to the question. For each dataset instance, we define a pointer $r$ to the visual region which the question or answer refer to, and compare it to the look at the model visual attention (summing up the overall attention the model gives to $r$). This metric allows us to evaluate the degree to which the model grounds its reasoning in the image, rather than just making educated guesses based on language priors or world tendencies. 

% in fact  indeed
We can see from the experiments that the attention models indeed mostly attend to the right and relevant regions in the image, with grounding scores of about 80\%. To verify the realiability of the metric, we further perform experiments with spatial features instead of the object-informed ones used by BottomUp \cite{bottomup} and MAC \cite{mac}, which lead to a much lower 43\% score, demonstrating that object-based features provide models with better granularity for the task, allowing them to focus on more pertinent regions than the coarser spatial features.

% validity and plausibility scores are quite high across all models (except those with no access the to question such as the CNN baseline), with plausibility somewhat lower than validity, as could be expected. We can conclude that the models manage to learn the scope of valid and plausible answers, a noticeable statistic of the dataset's question-conditional answer distribution. On the flip side, models indicate that for at least 10\% of the questions, models fail to even realize 

% As we can see in table \ref{table2}, while models manage to learn responding valid responses, which can be relatively easily identified by fitting answer distributions, they fail to provide plausible answers, which may require further degree of common-sense or world knowledge. The results also show that models frequently fail to be \textit{consistent}, replying with contradictory answers to equivalent or entailed questions. 

% The experiments show that all models except the CNN baseline (which cannot access the question) and the priors achieve very high validity scores -- 88 or higher. We can learn from this that the neural easily learn that scope of possible answers to a given question, which is a noticeable statistic of the data: the models can learn to reply with valid responses by modeling the dataset answer distribution conditioned on the question, without a need for further visual or semantic understanding.

 
% Second, the \textbf{validity} metric measures the extent to which a model's response is in the scope of theoretically-possible answers to a given question for at least some images. For instance, if a question asks whether a color of an apple is red or green, only these two alternative are valid answers. Indeed all models except the CNN baseline (which cannot access the question) and the most-common answer priors achieve very high validity scores -- 88 or higher. We can learn from this that the neural easily learn that scope of possible answers to a given question, which is a noticeable statistic of the data: the models can learn to reply with valid responses by modeling the dataset answer distribution conditioned on the question, without a need for further visual or semantic understanding.

%The \textbf{plausibility} metric goes further by checking whether the model's answer occurs with the object at least once in the whole dataset, \eg for a question about the color of an apple, \textit{red} and \textit{green} are plausible since there are such apples in the dataset scene graphs, but conversely, \textit{purple} is implausible. The original version of the paper considered an answer to be plausible if it occurs at least 20 times, but to make this measure more conservative, we lowered this threshold to 1. Consequently, the new plausibility scores are the following: much higher scores. 
% Other metrics that we use include \textit{Validity} and \textit{Plausibility}. The former measures whether the model response is in the scope the question defines, \eg responding with a color for a color question \etc., while the latter quantifies the degree to which the answer is reasonable, or makes sense given the question (\eg elephant usually do not eat, say, pizza).
% with

% Second, the \textbf{validity} metric 
% We can see that both validity and plausibility score are quite high for almost all models (except those that cannot access the question such as the CNN baseline). We can conclude that the models manage to learn the scope of valid and plausible answers to given questions, and so capture well at least the general tendencies of the dataset question-conditional answer distribution 
% Second, the \textbf{validity} metric measures the extent to which a model's response is in the scope of theoretically-possible answers to a given question for at least some images. For instance, if a question asks whether a color of an apple is red or green, only these two alternative are valid answers. Indeed all models except the CNN baseline (which cannot access the question) and the most-common answer priors achieve very high validity scores -- 88 or higher. We can learn from this that the neural easily learn that scope of possible answers to a given question, which is a noticeable statistic of the data: the models can learn to reply with valid responses by modeling the dataset answer distribution conditioned on the question, without a need for further visual or semantic understanding.

% Finally, the \textbf{plausibility} metric measures whether the model responses are reasonable in the real world or not making sense. For each open question about the attribute of an object, \textit{we check whether the model prediction occurs at least once as an attribute of the object over the whole dataset}. For instance, for a question about the color of an apple, we consider red and green as plausible since they occur as attributes for some scene graph within the dataset, and purple as implausible since there the dataset does not contain any purple apples. Similarly, we measure the plausibility of relations to occur with their subjects and objects. \textit{While this metric may not be fully precise especially for infrequent objects due to data scarcity issues, it may provide a good sense of the general level of world-knowledge the model has acquired}. The original version of the paper considered an answer to be plausible if it occurs at least 20 times, but to make this measure more conservative, we lowered this threshold to 1. Consequently, the new plausibility scores are the following: much higher scores. We can see that all models perform reasonably well on this metric, again demonstrating that the all methods that can access the questions manage to model the question-conditional answer distribution with good precision.

%\begin{figure}
%\centering
%\subfloat{\includegraphics[width=0.5\linewidth]{imgs/semcakeNew.pdf}}

%\subfloat{\includegraphics[width=0.67\linewidth]{imgs/sceneF.pdf}}
%\caption{\textbf{Top}: Distribution of GQA questions semantic length. \textbf{Bottom}: Performance as a function of the input representation. We encode the scenes through three different methods: spatial features produced by a standard pretrained CNN, object-based features generated by a faster R-CNN detector, and direct embedding of the scene graph semantic representation, equivalent to having perfect sight. We further experiment with both textual questions as well as their counterpart functional programs as input. We can see that the more semantically-imbued the representations get, the higher the accuracy obtained.}
%\label{plotss}
%\end{figure}

